On Scaling Data-Driven Loop Invariant Inference

Automated synthesis of inductive invariants is an important problem in software verification. Once all the invariants have been specified, software verification reduces to checking of verification conditions. Although static analyses to infer invariants have been studied for over forty years, recent years have seen a flurry of data-driven invariant inference techniques which guess invariants from examples instead of analyzing program text. However, these techniques have been demonstrated to scale only to programs with a small number of variables. In this paper, we study these scalability issues and address them in our tool oasis that improves the scale of data-driven invariant inference and outperforms state-of-the-art systems on benchmarks from the invariant inference track of the Syntax Guided Synthesis competition.

==> figures/code2inv-eval.tex <==
\begin{table}[t]
    \centering\relscale{0.95}%
    \def\arraystretch{1.05}%
    \begin{tabularx}{0.575\textwidth}{c | r | r}
        \toprule
        \textbf{\relscale{1.1} Tool} & \makecell{\bf Total Solved \\ \smaller{\bf (out of 133)}} & \makecell{\bf Unique Solved \\ \smaller{\bf (out of 92 unique)}} \\
        \midrule
        \codetoinv    & 106\,\textbf{*}               & --- \\
        \cvc          & 104\ \ \,                     & 70 \\
        \lig          & 97\ \ \,                      & 65 \\
        \lighe        & 109\ \ \,                     & 74 \\
        \oasis        & \textbf{121}\ \ \,            & \textbf{81} \\
        \bottomrule
    \end{tabularx}\vspace{0.5em}
    \caption{Results on 133 instances studied by \citet{nips18/si/code2inv} requiring reasoning over linear arithmetic.
             We allow a timeout of 300\,s for each instance with each tool.
             \textbf{*}\,See \cref{rem:code2inv}.\vspace{-0.5em}}
             %\fxtodo{wraptable}}
    \label{tab:resultsmain}
\end{table}

==> figures/lia-nia-eval.tex <==
\begin{table}[t]%
    \begin{subtable}[t]{0.475\textwidth}%
      \centering\relscale{0.95}%
      \def\arraystretch{1.05}%
      \begin{tabular}{ c | r }
        \toprule
        \textbf{Tool} & \textbf{Solved} \\
        \midrule
        \cvc          & 135 \\
        \lig          & 142 \\
        \lighe        & 144 \\
        \oasis        & \textbf{145} \\
        \bottomrule
      \end{tabular}
      \captionsetup{skip=0.5em}
      \caption{Results on 162 linear instances}
      \label{tab:resultslin}
    \end{subtable}\hfill%
    \begin{subtable}[t]{0.475\textwidth}%
      \centering\relscale{0.95}%
      \def\arraystretch{1.05}%
      \begin{tabular}{ c | r }
        \toprule
        \textbf{Tool} & \textbf{Solved} \\
        \midrule
        \cvc          & 6 \\
        \lig          & 7 \\
        \lighe        & 8 \\
        \oasis        & \textbf{10} \\
        \bottomrule
      \end{tabular}
      \captionsetup{skip=0.5em}
      \caption{Results on 18 non-linear instances}
      \label{tab:resultsnonlin}
    \end{subtable}
    \captionsetup{skip=0em}
    \caption{Results on 180 instances studied by \citet{cav19/padhi/hybrid-lig} requiring reasoning over linear and non-linear arithmetic.
             We allow a total timeout of 300\,s for linear, and 600\,s for non-linear instances.\vspace{-1.5em}}
\end{table}

==> figures/sampling-example.tex <==
\begin{center}
\begin{figure}
\begin{algorithmic}[1]\linespread{1}\selectfont
\FunctionX{\textnormal{pre}}{$x,y,z,size$}
    \State $(x = 0)$
\EndFunction
\FunctionX{\textnormal{trans}}{$x_{i},y_{i},z_{i},size_{i},x_{i+1},y_{i+1},z_{i+1},size_{i+1}$}
    \State \textsc{Or (}
    \State \hspace{\algorithmicindent} \textsc{And (}
    \State \hspace{\algorithmicindent} \hspace{\algorithmicindent}  $x_{i} < size_{i},$
    \State \hspace{\algorithmicindent} \hspace{\algorithmicindent} $x_{i+1} = x_{i} + 1,$
    \State \hspace{\algorithmicindent} \hspace{\algorithmicindent} $z_{i} \leq y_{i},$
    \State \hspace{\algorithmicindent} \hspace{\algorithmicindent} $size_{i+1} = size_{i},$
    \State \hspace{\algorithmicindent} \hspace{\algorithmicindent} $z_{i+1} = z_{i},$
    \State \hspace{\algorithmicindent} \hspace{\algorithmicindent} $y_{i+1} = z_{i}),$
    \State \hspace{\algorithmicindent} \textsc{And (}
    \State \hspace{\algorithmicindent} \hspace{\algorithmicindent} $x_{i} < size_{i},$
    \State \hspace{\algorithmicindent} \hspace{\algorithmicindent} $x_{i+1} = x_{i} + 1,$
    \State \hspace{\algorithmicindent} \hspace{\algorithmicindent} \textsc{Not}$(z_{i} \leq y_{i}),$
    \State \hspace{\algorithmicindent} \hspace{\algorithmicindent} $size_{i+1} = size_{i},$
    \State \hspace{\algorithmicindent} \hspace{\algorithmicindent} $z_{i+1} = z_{i},$
    \State \hspace{\algorithmicindent} \hspace{\algorithmicindent} $y_{i+1} = y_{i})$
    \State )
\EndFunction
\FunctionX{\textnormal{post}}{$x,y,z,size$}
    \State \textsc{Or (}$(size > 0), (z \geq y)$)
\EndFunction
\end{algorithmic}
\caption{An example \textsc{Smt} instance with $pre(\pstate)$, $trans(\pstate_i, \pstate_{i+1})$ and $post(\pstate)$ functions. Here, program state $\sigma$ is a 4-tuple of assignments to the variables $(x, y, z, size)$. The $trans$ function encodes 
the loop body --- the program state changes from $\pstate_i$ to $\pstate_{i+1}$ after one execution of the function.}
\label{fig:sampling_ex}
\end{figure}
\end{center}


==> figures/time-sample.tex <==
\begin{table}[t!]
    \centering\relscale{0.95}%
    \def\arraystretch{1.05}%
    \begin{tabular}{c | c | r | r}
        \toprule
        \textbf{Benchmark} & \textbf{Statistic} & \makecell{\bf Iteration \\ \bf Count} & \makecell{\bf Running \\ \bf Time (s)} \\
        \midrule
         45 out of 92 & Min & 1 &  1.4\\
         linear instances   & Median &  2                      &  5.1 \\
         \citep{nips18/si/code2inv} & Max & 164 &  135.3 \\ \midrule
         79 out of 162  & Min & 1 &  1.1 \\
         linear instances   & Median & 3                    &  2.8 \\
         \citep{cav19/padhi/hybrid-lig} & Max & 236 &  225.4 \\ \midrule
         8 out of 18 & Min & 1 & 2.6 \\
         non-linear instances   & Median & 1                 &  9.7 \\
         \citep{cav19/padhi/hybrid-lig}& Max & 9 & 41.5 \\
        \bottomrule
    \end{tabular}\vspace{0.5em}
    \caption{Number of iterations and the wall-clock time required by \oasis{} to solve the benchmarks.
             The statistics are computed on the instances that required at least one invocation of the ILP solver,
             \ie at least one \textsc{Learn} call from the \textsc{Infer} algorithm in \cref{fig:loopinvgen}.\vspace{-1.5em}}
    \label{tab:resultstime}
\end{table}

==> figures/unique.tex <==
\begin{table}[h!]
\centering
 \begin{tabular}{|c c|} 
 
 \hline
 \textbf{\relscale{1.1} Tool} & \makecell{\bf Solved} \\ 
 \hline\hline
  \cvc & 0\\
  \hline
 \dsynth & 11 \\ 
 \hline
 \lig & 1\\
 \hline
 \oasis & 13\\
 \hline

 \end{tabular}
 \caption{Uniquely solved benchmarks by each tool.}
\label{table:unqiue}
\end{table}

==> sections/plots.tex <==
 %\begin{center}
    \begin{figure}
    \centering
     \caption{Comparison between the number of variables in the solution of \unconfounded{} instances, variables in the corresponding \confoundedone{} variant of the benchmark and  variables used by \oasis{} for invariant inference. 23 benchmarks out of 83 benchmarks which \oasis{} solves have been ignored as they have post condition as their solution. }
     \label{fig:conf_one}
    \includegraphics[width=\textwidth,height=0.90\textheight,keepaspectratio]{conf1.png}
    
    \end{figure}
    
    \begin{figure}
    \centering
     \caption{Comparison between the number of variables in the solution of \unconfounded{} instances, variables in the corresponding \confoundedfive{} instances and  variables used by \oasis{} for invariant inference. 6 benchmarks out of 66 benchmarks which \oasis{} solves have been ignored as they have post condition as their solution.}
     \label{fig:conf_five}
    \includegraphics[width=\textwidth,height=0.90\textheight,keepaspectratio]{conf5.png}
     
     \end{figure}
%\end{center}
%add captions, take aways

%take-away, The variable statistics table and table 1 clearly indicates that as the problem becomes complex i.e, the number of variables increase, there is a drop in the performance of the tools. Our active learning algorithm helps in reducing the numbers of variables given to the inference engine and hence reducing the complexity of the problem. Average compression is 3.907 for confounded5 benchmarks and 2.48 for confounded1 bechmarks


==> sections/subroutines.tex <==


% \begin{algorithmic}[1]\linespread{1}\selectfont
% \Func{\textnormal{\sc \generatedata}}{$pre(x),trans(x_{i},x_{i+1}),post(x),depth$}
%     \State $T \gets \textnormal{\sc ConvertToDNF}(trans)$   \Comment{returns a set of dijuncts in trans expression}
%     \State $n \gets length(T)$
%     \State $posState \gets  \{\}$
%     \State $negState \gets  \{\}$
%     \For{$d \gets 1$ to $depth$}
%         \State $permutations \gets T^\times d$ \Comment{get all possible permutations of trans disjuncts of depth d} 
%         \For {$perm \in permutations$} 
%             \For{$(trans_{1},trans_{2},...,trans_{d}) \in perm$}
%                 \State $checkPos \gets pre(x_{0}) \wedge trans_{1}(x_{0},x_{1}) \wedge .. trans_{k}(x_{d-1},x_{d})$
%                 \State $checkNeg \gets trans_{1}(x_{0},x_{1}) \wedge ... trans_{d}(x_{d-1},x_{d}) \wedge \neg(post(x_{d}))$ 
%                 \If{$checkPos = SAT$}
%                     \State $posState \gets posState \cup x_{d}$
%                 \EndIf
%                 \If{$checkNeg = SAT$}
%                     \State $negState \gets posState \cup x_{0}$
                
%                 \EndIf
%             \EndFor
%         \EndFor
    
%     \EndFor
%     \State $data \gets posState \cup negState $
%     \State \Return $data$
% \EndFunc
% \end{algorithmic}

\begin{algorithmic}[1]\linespread{1}\selectfont
\Func{\textnormal{\sc \generateselecdata}}{$pre(\pstate),trans(\pstate_{i},\pstate_{i+1}),post(\pstate),expr,depth$}
    \State $T \gets \textnormal{\sc ConvertToDNF}(trans(\pstate_{i},\pstate_{i+1}))$   \Comment{returns a set of dijuncts in trans expression}
    % \State $n \gets length(T)$
    \State $posState \gets  \{\}$
    \State $negState \gets  \{\}$
    \If{$expr$}
        \State $pexpr \gets expr$
        \State $nexpr \gets \neg(expr)$
    \Else
        \State $pexpr \gets \true$
        \State $nexpr \gets \true$
    \EndIf
    \For{$d \gets 1$ to $depth$}
        \State $permutations \gets T^\times d$ 
        \For {$perm \in permutations$} \Comment{get all possible permutations of trans disjuncts of depth d}
            \For{$(trans_{1},trans_{2},...,trans_{d}) \in perm$}
                \State $checkPos \gets pre(\pstate_{0}) \wedge trans_{1}(\pstate_{0},\pstate_{1}) \wedge .. trans_{d}(\pstate_{d-1},\pstate_{d}) \wedge nexpr$
                \State $checkNeg \gets trans_{1}(\pstate_{0},\pstate_{1}) \wedge ... trans_{d}(\pstate_{d-1},\pstate_{d}) \wedge \neg(post(\pstate_{d})) \wedge pexpr$ 
                \If{$checkPos = SAT$}
                    \State $posState \gets posState \cup \pstate_{d}$
                \EndIf
                \If{$checkNeg = SAT$}
                    \State $negState \gets negState \cup \pstate_{0}$
                
                \EndIf
            \EndFor
        \EndFor
    
    \EndFor
    \State $data \gets posState \cup negState $
    \State \Return $data$
\EndFunc
\end{algorithmic}

%Edited
% \begin{algorithmic}[1]\linespread{1}\selectfont
% \Func{\textnormal{\sc \activelearn}}{$pre(x),trans(x_{i},x_{i+1}),post(x),depth$}
%   %\Comment{add exhaustive enumeration code}
%   \State $data \gets {\textnormal{\sc\generateselecdata}}(pre(x),trans(x_{i},x_{i+1}),post(x),expr)$
%     \State $expr \gets {\textnormal{\sc \learn}}(data)$
%     \State $relevantVars \gets \textnormal{\sc TransitiveClosure}(expr)$ \Comment{get the transitive closure of vars in expr}
%     \State \Return $expr,relevantVars$
% \EndFunc
% \end{algorithmic}


\begin{algorithmic}[1]\linespread{1}\selectfont
\Func{\textnormal{\sc \getrelevantvars}}{$data$}
  % \State $data \gets \textnormal{\sc \generateselecdata}(pre(\pstate),trans(\pstate_{i},\pstate_{i+1}),post(\pstate),expr,depth)$
    \State $expr \gets {\textnormal{\sc \learn}}(data)$
    \State $relevantVars \gets \textnormal{\sc TransitiveClosure}(expr)$ \Comment{get the transitive closure of vars in expr}
    \State \Return $expr,relevantVars$
\EndFunc
\end{algorithmic}

